The SPECIAL-K Personal Data Processing Transparency and Compliance Platform

The European General Data Protection Regulation (GDPR) brings new challenges for companies who must ensure they have an appropriate legal basis for processing personal data and must provide transparency with respect to personal data processing and sharing within and between organisations. Additionally, when it comes to consent as a legal basis, companies need to ensure that they comply with usage constraints specified by data subjects. This paper presents the policy language and supporting ontologies and vocabularies, developed within the SPECIAL EU H2020 project, which can be used to represent data usage policies and data processing and sharing events. We introduce a concrete transparency and compliance architecture, referred to as SPECIAL-K, that can be used to automatically verify that data processing and sharing complies with the data subjects consent. Our evaluation, based on a new compliance benchmark, shows the efficiency and scalability of the system with increasing number of events and users.

==> sections/fullevaluation.tex <==
\section{Evaluation}
\label{s:evaluation}

In this section, we use the SPECIAL compliance benchmark to evaluate our SPECIAK-K platform. We report the averaged results of 3 independent executions. All experiments were executed on a cluster consisting of 10 nodes. Although, it is expected that large-scale companies could provide more computational resources, this installation: (i) can serve many data-intensive scenarios as we will show in the results; and (ii) is meant to provide clear guidelines on the scalability of the platform, which can help to plan future installations and evaluations. The characteristic of the cluster are presented in \emph{Table} \ref{t:cluster}.

\begin{table}[t!]
\center
\caption{Characteristic of the cluster}
\scriptsize
\begin{tabular}{p{2.5cm}p{4cm}}
\toprule
Number of Nodes & 10 \\
CPUs & Each node consists of 4 CPUs per machine (2 cores per CPU)\\
Memory & 16 GB per node \\
Disk Space & 100 GB per node \\
Operating System & CoreOS 2023.5.0 (Rhyolite) \\
Replication Factor & 2. As mentioned this implies that data is written to 2 nodes, enhancing fault-tolerance at the cost of additional space requirements and a minimum time overhead \\
\hline
\end{tabular}
\label{t:cluster}
\normalsize
\end{table} 


\subsection{Scaling the Compliance Checking Process}
\label{s:scaling}

Before delving into the concrete results on the the SPECIAL compliance benchmark tasks, we present here a first study on the scalability of the system with respect to the number of processes executing compliance checking. 
%
Topics in Kafka are divided into partitions, which are the actual log structures persisted on disk. The number of partitions establishes an upper limit to how far the processing of
records can be scaled out, given that a partition can only be assigned to a single consumer (in a consumer group). Thus, the total number of partitions of the application log topic will decide how many instances of the compliance checker can process the data in parallel.
%
Given the available resources of the cluster, we decided to set up 10 partitions, which puts an upper limit of 10 compliance checkers running in parallel. 
%
As a first evaluation, we show how the system behaves with increasing compliance checkers running in parallel. We perform the test in a streaming and batch processing scenario. 

\begin{figure}[t]
  \begin{center}
    \includegraphics[width=.5\textwidth]{images/latencies-c21-1ms-differentCheckers.pdf}
     \caption{\label{fig:latencies-c1-differentCheckers}Median and average latencies with increasing number of compliance checkers}
  \end{center}
\end{figure}

\begin{figure}[t]
  \begin{center}    
    \includegraphics[width=.5\textwidth]{images/c21-1ms-checks-percentile-1-3-5-10.pdf}
 \caption[Latencies (in 95\% percentile) with increasing number of compliance checkers]{\label{fig:percentile-1-3-5-10}Latencies (in 95\% percentile) with increasing number of compliance checkers (1, 5, 10 checkers)}
 
    \includegraphics[width=.5\textwidth]{images/c21-1ms-checks-percentile-5-10.pdf}
        \caption[Latencies (in 95\%, 75\% and 50\% percentile) with increasing number of compliance checkers]{\label{fig:percentile-1-10}Latencies (in 95\%, 75\% and 50\% percentile) with increasing number of compliance checkers (1, 10 checkers)}
  \end{center}
\end{figure}

\begin{figure}[t]
  \begin{center}
    \includegraphics[width=.5\textwidth]{images/cpu-c21-1ms-differentCheckers.pdf}
  \caption[CPU usage with increasing number of compliance checkers]{\label{fig:CPU-usage-1-3-5-10}CPU usage (in \%) with increasing number of compliance checkers}
  
    \includegraphics[width=.5\textwidth]{images/memory-c21-1ms-differentCheckers.pdf}
    \caption[Memory usage with increasing number of compliance checkers]{\label{fig:memory-usage-1-3-5-10}Memory usage (in GB) with increasing number of compliance checkers}
      \end{center}
\end{figure}

\subsection{Streaming}
\label{ss:scaleStreaming}

For this scenario, we evaluate the streaming task \emph{C-T4-4} from the SPECIAL compliance benchmark, shown in Table \ref{t:compTasks}. Note that the task considers a stream of 1,000 users, where each user generates 1 event every second. That is, we evaluate an event stream that, on average, generates \emph{1 event every 1ms}, producing a total of 1,200,000 events. Given that we expect a performance on the level of ms per check, the streaming flow is close to the limit of one compliance checker.

Figure \ref{fig:latencies-c1-differentCheckers} shows the median and average latency (in milliseconds, with logarithm scale) with different number of compliance checkers in parallel, ranging from 1 to 10 (with 10 being the upper limit defined by the number of partitions as explained above). Note that the median is usually preferred to the average given that the latency distribution can be skewed. 
%
Results show that the (median) latency is always at the level of milliseconds (in particular, less than 2.5 ms), with a noticeable improvement when more compliance checkers are running in parallel, providing a \emph{stable latency of 1.5 ms}. As expected, the slightly higher average figures denote the expected skewed distribution. 

Given this behaviour, we inspect the percentile latency, i.e, the value at which a certain percentage of the data is included. Figure \ref{fig:percentile-1-3-5-10} represents (in milliseconds and logarithm scale) the latency at 95\% percentile, using 1, 5 or 10 parallel checkers. For instance, a value of `100' ms means that 5\% of the events have a latency greater than or equal to `100' ms. 
%
The distribution of 95\% percentiles first shows an initial \emph{warm-up} effect, with higher latencies until the first 10,000 events. Then, the latencies are stable with 1-2 ms in all cases, even at the high streaming rate of 1 event every ms. That is, in general, only 5\% of the events can experience latencies over 1-2 ms. As expected, latencies are slightly greater if only 1 checker is used. It is worth noting that the evaluation uncovered a recurrent peak with 5 checkers around 20,000 events, which is subject of future inspection.

Figure \ref{fig:percentile-1-10} completes this analysis, depicting 50, 75 and 95\% percentiles for the extreme cases of having 1 or 10 checkers in place. In this case, the 50 and 75 \% percentiles are close to the 95\%, which reflects that most of the data is in the range of the 95\% percentile. 

In the following, we evaluate the CPU usage (in percentage) and memory usage (in GBs) with increasing number of parallel compliance checkers (1, 5 and 10), shown in Figures \ref{fig:CPU-usage-1-3-5-10} and \ref{fig:memory-usage-1-3-5-10} respectively. We report the average and the maximum number. 
%
Results show that, thanks to latest improvements in the third release of the platform, (i) memory usage increases sublinearly (and remains under 2 GBs) as more parallel compliance checkers are running in parallel, and (ii) CPU consumption remains stable around 50\%, with no major influence of the number of checkers. Both results show that Kafka is able to optimise the use of resources and to adapt to the number of parallel checkers.  In addition, it is worth mentioning that Kafka is able to add compliance checkers dynamically. 

Overall, although different application scenarios can have highly demanding real-time requirements, we expect that these figures, e.g. serving a 95\% percentile latency of 1-2ms with an event stream of 1 event every 1ms, can cover a wide range of real-world scenarios. Recall that the limit of 10 parallel compliance checkers is solely bounded to the number of partitions in the installation, which depends on the resources of the cluster.

\begin{figure}[t]
  \begin{center}
    \includegraphics[width=.5\textwidth]{images/throughput-differentCheckers.pdf}
 
  \caption[Total batch throughput by the compliance checker with increasing number of compliance checkers]{\label{fig:batch-throughput-1-3-5-10}Total batch throughput (in events/s) by the compliance checker with increasing number of compliance checkers}
  
    \includegraphics[width=.5\textwidth]{images/throughput-distribution-1-3-5-10.pdf}
   \caption[Distribution of batch throughput by the compliance checker with increasing number of compliance checkers]{\label{fig:batch-throughput-distribution-1-3-5-10}Distribution of batch throughput (in events/s) by the compliance checker with increasing number of compliance checkers}
   \end{center}

\end{figure}  
\begin{figure}[t]
  \begin{center}
    \includegraphics[width=.5\textwidth]{images/latencies-c1-10ms-unions.pdf}
  \caption{\label{fig:t1-complexPoliciesMedian}Median and average latencies with increasing complex policies}
    \end{center}
\end{figure}
  
\begin{figure}[t]
  \begin{center}
    \includegraphics[width=.5\textwidth]{images/c1-1check-percentile-policies-1-10-30.pdf}

 \caption{Latencies (in 95\% percentile) with increasing complex policies}
  \label{fig:t1-complexPoliciesLatency}
    \end{center}
\end{figure}  
  
\begin{figure}[t]
  \begin{center}
    \includegraphics[width=.5\textwidth]{images/latencies-c8-c11-users.pdf}
  \caption{Median and average latencies with increasing number of users}
  \label{fig:t2-Median}
    \end{center}
\end{figure}

\begin{figure}[t]
  \begin{center}
    \includegraphics[width=.5\textwidth]{images/latencies-c8-c11-users-percentile.pdf}

 \caption{Latencies (in 95\% percentile) with increasing number of users}
  \label{fig:t2-Latency}
    \end{center}
\end{figure}  

\begin{figure}[t]
  \begin{center}
    \includegraphics[width=.5\textwidth]{images/latencies-c18-c22-rate.pdf}
  \caption[Median and average latencies with increasing generation rates]{\label{fig:t4-rateMedian}Median and average latencies with increasing generation rates. The rate refers to events per user, with 1K users}
  
   \includegraphics[width=.5\textwidth]{images/latencies-c18-c22-rate-percentile.pdf}
    \caption[Latencies (in 95\% percentile) with increasing generation rates]{\label{fig:t4-rateLatency}Latencies (in 95\% percentile) with increasing generation rates. The rate refers to events per user, with 1K users}
    \end{center}
\end{figure}

\begin{figure}[t]
  \begin{center}
    \includegraphics[width=.5\textwidth]{images/cpu-c18-c22-rate.pdf} 
  \caption[CPU usage for compliance checking with increasing generation rate]{CPU usage (in \%) for compliance checking with increasing generation rate (1K users)}
  \label{fig:CPU-usage-t4-rates}
    \end{center}
\end{figure}  

\begin{figure}[t]
  \begin{center}
    \includegraphics[width=.5\textwidth]{images/throughput-batch-c23-25.pdf}
  \caption[ Total batch compliance checking  throughput with increasing number of compliance checkers]{\label{fig:batch-throughput-c23-25} Total batch compliance checking  throughput (in events/s) with increasing number of compliance checkers}
    \includegraphics[width=.5\textwidth]{images/throughput-batch-distribution-c23-25.pdf}
  \caption[Distribution of batch compliance checking throughput with different users and work load]{\label{fig:batch-throughput-distribution-c23-25}Distribution of batch compliance checking throughput (in events/s) with different users and work load. We consider 1000 events per user}  
    \end{center}
\end{figure}   

\subsection{Batch processing}
\label{ss:scaleBatch}

As stated in choke point CCP6, the system must also deal with performant compliance checking in batch. Thus, we repeat the previous analysis looking at different number of compliance checkers for the case of batch processing. To this aim, we evaluate the batch task \emph{C-T5-2} from the SPECIAL compliance benchmark, shown in Table \ref{t:compTasks}. This task considers 1,000,0000 events that are already loaded in the system. Given that we process events in batch, we inspect the provided throughput (processed events per seconds) using an increasing number of compliance checkers.

Figure \ref{fig:batch-throughput-1-3-5-10} shows the total batch throughput (in events/s) for 1, 5 and 10 compliance checkers running in parallel. Similarly to the streaming scenario, the performance is improved significantly as more instances are running concurrently. In this case, we can observe a sublinear behaviour, where the throughput ranges from 1796 events/s with 1 checker to 2523 events/s with 10. The difference between 5 and 10 checkers is negligible.

Figure \ref{fig:batch-throughput-distribution-1-3-5-10} shows the distribution of batch throughput (in events/s) across time, for 1, 5 and 10 compliance checkers. Results are consistent with the throughput reported above, showing  a general constant behaviour and a better performance with 5 and 10 checkers running in parallel.
  
\begin{table*}[t!]
\center
\caption[Space requirements with increasing generation rate]{Space requirements (MB) with increasing generation rate.}
\scriptsize
\begin{tabular}{llrr}
\toprule
{\bf \# Users} & {\bf Event Rate (per user)} & {\bf \# Events} & {\bf Disk Space (MB)} \\
\hline
1,000 & 1 ev./60s & 20,000 &  819 \\
1,000 & 1 ev./30s & 40,000 &  1,563 \\
1,000 & 1 ev./10s & 120,000 &  1,954 \\
1,000 & 1 ev./1s & 1,200,000 &  5,355\\
1,000 & 1 ev./100ms & 12,000,000 &  59,664\\

\hline

\end{tabular}
\label{t:space}
\normalsize
\end{table*} 


\subsection{Results on STC-bench Compliance Tasks}
\label{s:results}

This section provides results on the the SPECIAL compliance benchmark tasks, shown in Section \ref{s:benchmark}. Rather than showing a complete evaluation on an optimised and performant infrastructure, we focus on testing an installation of the SPECIAL platform and pinpointing good spots for optimisation. 
%
We limit our scope to the functionality provided by the current third release of the SPECIAL platform and the scaling capabilities of the infrastructure. In the following we present the results for all the compliance tasks (\emph{C-T1} to \emph{C-T5} from Table \ref{t:compTasks}). We disregard \emph{C-T3} as no significant differences were found in our tests and we opt for a more realistic random generation of policies. 

\subsubsection{C-T1: Different Complexities of Policies}
\label{ss:t1}

Recall that this task regards the behaviour of the system in a streaming scenario (at 1 event/10s per user and 1K users) when different complexities of policies, measured as the number of union policies, are considered. In this scenario, we make use of 1 compliance checker in order to isolate the performance of one instance. We also compare the implementation of the Hermit reasoner with our engine PLReasoner.

Figure \ref{fig:t1-complexPoliciesMedian} shows the median and average latencies (in milliseconds) with 1, 10 and 30 union policies. Results show that the median \emph{latency ranges between 1.5-5 ms}, with relatively small differences as the number of union policies grows, except for the union of 30 policies. In this case, the higher number of union policies allows Hermit to quickly find a match (1.5 ms). As for the comparison of reasoners, Hermit seems to slightly outperform PLReasoner in the scenario under test. Nonetheless, when both reasoners are run in isolation, the tailored PLReasoner engine is several times faster than Hermit \cite{specialD3.5}. A first analysis shows that different parsing and deserialisation of policies can affect the times of PLReasoner in the SPECIAL platform. In addition, our isolated study generally considers richer and more complex policies than STC-bench, also including different time intervals (for the duration of the storage).


Finally, the higher figures for the average latency again denote a skewed distribution. Thus, we inspect the latency at 95\% percentile (the value at which 95\% of the data is included), depicted in Figure \ref{fig:t1-complexPoliciesLatency} for 1, 10 and 30 policies. The distribution shows that, in all scenarios, the latency at 95\% percentile is stable after the warm-up, with small differences with more union policies. Results also show that only 5\% of the events can experience latencies over 5 ms. 


\subsubsection{C-T2: Increasing Number of Users}
\label{ss:t2}

The second task in the SPECIAL compliance benchmark focuses on evaluating the scalability of the system with increasing number of users, from 100 to 1 million. These users are considered to be generating events in parallel, each of them at a rate of 1 event every 10 seconds. In the following evaluation, we study the first four subtasks, covering up to 100,000 users given the characteristics of the experimental infrastructure. Note that serving 100,000 users at the aforementioned rate already implies to manage a stream of 10,000 events every second. In this scenario, we consider 10 compliance checkers running in parallel in order to cope with such demand. As mentioned above, we expect that this evaluation can serve as a baseline to shed light on the potential of the SPECIAL platform, guiding our current efforts. 


Figure \ref{fig:t2-Median} shows the median and average latencies for 100-100,000 users. Results show that the system is able to provide a median latency of less than 1ms with 1,000 users (each user with 1 event every 10 seconds, hence overall the system receives 1 event every 10 ms simultaneously), and 1.6ms with 10,000 users (overall, 1 event very ms). However, with 100,000 users, the current infrastructure needs to manage 1 event every 0.1ms (less than the checking time of 1ms), which causes delays of several seconds. 

In order to highlight potential worst-case scenarios, we represent the latency at 95\% percentile in Figure \ref{fig:t2-Latency}. Note that an increasing number of users results in more events, hence the different number of events in each scenario. As expected, results show two different scenarios. On the one hand, a number of users between 100-10,000 results in a \emph{95\% percentile around 1 ms}, with an initial warm-up step that produces higher latencies. On the other hand, a higher number of users (100,000) leads to increasing latencies as the number of events grows, i.e. events are queued for several seconds. The main reason is that the number of compliance checkers (10, given the amount of computational resources in the cluster) cannot cope with the overall actual ratio of 10,000 events every second. Given that Kafka is able to optimise and adapt to the number of parallel checkers, which is solely limited by the number of partitions in the cluster, hence a more powerful infrastructure could cope with a greater number of users.


\subsubsection{C-T4: Increasing Data Generation Rates}
\label{ss:t4}

This task evaluates the performance of the system with increasing streaming rates. We consider 10 compliance checkers running in parallel in order to try to cope with the biggest rates in the defined tasks.

Figure \ref{fig:t4-rateMedian} represents the median and average latencies (in milliseconds and logarithm scale), while the latency at 95\% percentile is shown in Figure \ref{fig:t4-rateLatency} (in logarithm scale). Several comments are in order. First, note that the median values in Figure \ref{fig:t4-rateMedian} are consistent with our previous latency measures, obtaining values between 1-2ms for rates up to 1 ev/s (per user). Then, as expected, the median latency increases up to several seconds at the highest rate of 1 ev/100ms per user, that is, the system receives a total of 1 ev/0.1ms.


The huge skewed distribution for the highest rate is revealed by the 95\% percentile shown in Figure \ref{fig:t4-rateLatency}. Note that we fix the benchmark time at 20 minutes, so more events are generated with increasing generation rates. Results shows that, the latency reaches a stable stage for rates up to 1 ev/1s per user, i.e. a total of 1 ev/1ms. In contrast, the latency at 95\% percentile grows steadily for streams at 1 ev/100ms per user. This fact shows that the current installation cannot cope with such high rates and new events have to queue until they can be processed. The maximum latency reaches 17 minutes for 12 million events. 

Finally, in this case, we also inspect the CPU usage and the overall disk space of the solution. The CPU usage (in percentage) is represented in Figure \ref{fig:CPU-usage-t4-rates}. As expected, the results show that the CPU usage increases (but sublinearly) with the generation ratio. The disk space requirements are given in Table \ref{t:space}. It is worth mentioning that the disk space depends on multiple factors, such as the individual size of the randomly generated events, the aforementioned level of replication, the number of nodes and the level of logging/monitoring in the system. The reported results already show the log compaction feature of Kafka as, on average, less bytes are required to represent each of the events with increasing event rates. 

\subsubsection{C-T5: Batch Performance}
\label{ss:t5}

Recall that this task considers a batch processing scenario, i.e. events are already loaded in the system,  with increasing number of events and users. In this evaluation, we consider the first three subtasks, testing up to 10 million events\footnote{Note that the system is able to generate and process an arbitrary number of events in batch. Further results can be found in our companion website.} (considering 100K events per user). We inspect the provided throughput (processed events per seconds) using an increasing number of compliance checkers. As in previous cases, we here consider 10 compliance checkers running in parallel.

Figure \ref{fig:batch-throughput-c23-25} shows the total batch throughput (in events/s) for 100K, 1M and 10M events. The total throughput increases with the number of events, being over 474 processed events/s in all cases, with a maximum of 3,489 events/s in the case of 10M events. 

Finally, Figure \ref{fig:batch-throughput-distribution-c23-25} looks at the distribution of the throughput for the case of 1M and 10M events. Both cases shows similar initial figures, with increased performance around 4M events.  






==> sections/specialK.tex <==


